Fundamental groups of compact Kahler varieties with nef anti canonical bundle

It is proved by M. Paun (1997, 2017) that the fundamental group of a compact Kahler manifold X is almost Abelian if the anti-canonical bundle -KX is nef. In this paper, we apply the recent geometric analytic theory of Kahler spaces developed by Guo-Phong-Song-Sturm to study fundamental groups of mildly singular compact Kahler varieties. We first extend Paun's result to log canonical pairs (X,Delta) with smooth X and nef -(KX+Delta) as well as to compact Kahler manifolds X with pseudo-effective -KX under a suitable assumption on the singularities of c1(-KX). We further prove that, for a 3-dimensional log canonical pair (X,\Delta) with X being klt, pi 1(X) is almost Abelian if -(KX+\Delta) is nef. Moreover, as one of the main ingredients for the proof of these results, we establish the surjectivity of the Albanese maps of compact normal complex varieties X in Fujiki class C that admits an effective R-divisor \Delta such that the pair (X,\Delta) is log canonical with nef anti-log canonical divisor -(KX+\Delta).This generalizes the corresponding theorems for projective varieties (Zhang, 2005), for klt pairs (Matsumura-Wang-Wu-Zhang, 2025) and for log smooth case (Fu-Han-Zou, 2025)

==> abelianity.tex <==
\section{Almost Abelianity of \texorpdfstring{$\pi_1(X)$}{text}}
In this section we give the proof of {\hyperref[thm:main1]{Theorem \ref*{thm:main2}}, preciesly, we show that for normal projective variety $X$ with lt singularities and nef anticanonical divisor, its fundamental group $\pi_1(X)$ is almost Abelian. Indeed, the theorem can be deduced immediately from {\hyperref[thm:main1]{Theorem \ref*{thm:main1}} and the following result of F. Campana:
\begin{proposition}[{\cite[Corollaire 3.1]{Cam95}}]
\label{prop:Alb_surj_pi1}
Let $Y$ be a compact K\"ahler manifold such that the Albanese map of $Y$ is surjective, then the nilpotent completion of $\pi_1(Y)$ is Abelian.
\end{proposition}

For the convenience of the readers, we will give the proof of the proposition by closely following the argument in \cite{Cam95}, which was written in French. We attempt to add clarification and explanations to the presentation. First recall some notions from group theory: let $G$ be a group, and let 
\[
G=G_0\supseteq G_1\supseteq \cdots\supseteq G_i \supseteq G_{i+1}\supseteq\cdots
\]
be the central series of $G$, i.e. we inductively define $G_{i+1}:=[G,G_i]$. And we put $G_{\infty}:=\bigcap_{i\geqslant 1}G_i$. For any $n\in\Z_{>0}\cup\{\infty\}$, we set $G'_n:=\sqrt{G_n}$, here for any subset $S\subseteq G$ we define 
\[
\sqrt S:=\left\{g\in G\;\big|\;g^n\in S\right\}.
\]
The \emph{$($torsion free$)$ nilpotent completion} of $G$ is defined to be $G^\nilp:=G/G'_\infty$\,. The proof of {\hyperref[thm:main2]{Theorem \ref*{thm:main2}}} is based on the following characterization due to J. Stallings:

\begin{theorem}[{\cite[Theorem 3.4]{Sta65}}]
\label{thm:Stallings}
Let $f:G\to H$ be a group morphism. Assume that $H_1(f): H_1(G,\Q)\to H_1(H,\Q)$ is an isomorphism and $H_2(f): H_2(G,\Q)\to H_2(H,\Q)$ is surjective. Then 
\begin{itemize}
\item[\rm(a)] the induced morphism $f_k: G/G'_k\to H/H'_k$ is injective for $k\in\Z_{>0}\cup\{\infty\}$ and is of finite index for $k\in\Z_{>0}$\,$;$
\item[\rm(b)] if $f$ is surjective, then $f_k$ is an isomorphism for each $k\in\Z_{>0}\cup\{\infty\}$.
\end{itemize}
\end{theorem}
\begin{proof}[Sketch of the proof]
The theorem can proved by induction combining with the following exact sequence established in \cite[Theorem 2.1]{Sta65}: 
\[
H_2(G) \to H_2(G/N) \to N/[G,N] \to H_1(G) \to H_1(G/N) 
\]
where $N\subseteq G$ is normal subgroup, and this sequence is functorial with respect to $f:(G,N)\to (G',N')$ where $f: G\to G'$ is a group morphism such that $f(N)\subseteq N'$. 
\end{proof}


Now let us turn to the proof of {\hyperref[prop:Alb_surj_pi1]{Proposition \ref*{prop:Alb_surj_pi1}}}. Indeed, we will prove a stronger result; in order to state it, let us first set up some notations: let $Y$ be a compact K\"ahler manifold and $\alb_Y: Y\to\Alb_Y$ be the Albanese map of $Y$, let $W$ be a desingularization of the image of $\alb_Y$. Take an elimination of indeterminacies $Y'\to W$ of $\alpha: Y\dashrightarrow W$ with the natural (birational) morphism $\mu:Y'\to Y$. Since $\mu$ induce an isomorphism on fundamental groups, we may assume that $\alpha$ is an (everywhere defined) morphism. 
%and since $\alb_{Y'}=\alb_Y\circ\mu_Y$, thus up to replacing $Y$ and $W$ by $Y'$ and $W'$ respectively, we may assume that $W$ is smooth (thus a compact K\"ahler manifold). 
We set $G:=\pi_1(Y)$ and $H:=\pi_1(W)$ and $\alpha$ induces a group morphism $\alpha_\ast:G\to H$. In the sequel we will prove the following:
\begin{theorem}[{\cite[Th\'eor\`eme 2.1]{Cam95}}]
\label{thm:Campana}
The induced morphism $\alpha_{\ast,n}:G/G'_n\to H/H'_n$ is injective for $n\in\Z_{>0}\cup\{\infty\}$ and is of finite index for $n\in\Z_{>0}$\,. Moreover, if $\alpha_\ast$ is surjective, then $\alpha_{\ast,n}$ is an isomorphism for each $n\in\Z_{>0}\cup\{\infty\}$.
\end{theorem}

\begin{proof}
In view of {\hyperref[thm:Stallings]{Theorem \ref*{thm:Stallings}}}, we just need to check that the following two conditions hold:
\begin{itemize}
\item[(i)] $H_1(\alpha):H_1(G,\Q)\to H_1(H,\Q)$ is an isomorphism; 
\item[(ii)] $H_2(\alpha): H_2(G,\Q)\to H_2(H,\Q)$ is surjective.
\end{itemize} 
To this end, we need to associate the cohomology of a complex variety (or more generally, a cell complex) to the (group) homology of its fundamental group. This can be done by the following construction: 

Let $K$ be a connected cell complex, by adding cells of dimension $\geqslant 3$ to $K$ we can construct an aspherical complex $K'$ so that $K$ is embedded into $K'$. From the construction we see that the higher homotopy groups of $K'$ are all vanishing, hence $K'=K(\pi_1(K),1)$ the Eilenberg-Maclane space of $\pi_1(K)$, in particular $H_n(K')\simeq H_n(\pi_1(K))$ for any $n$. Since $K'\backslash K$ does not contain any cell of dimension $\leqslant 2$, it follows that the natural morphism $H_1(K)\to H_1(K')$ is an isomorphism and $H_2(K)\to H_2(K')$ is surjective by looking at the homology sequence of the pair $(K',K)$:
\[
H_2(K)\to H_2(K')\to \underbrace{H_2(K',K)}_{=0}\to H_1(K)\to H_1(K')\to \underbrace{H_1(K',K)}_{=0}\to 0.
\]
Hence $H_1(K)\simeq H_1(\pi_1(K))$ and $H_2(K)\twoheadrightarrow H_2(\pi_1(K))$. 

Now (i) follows from the construction of the Albanese map: the morphism of homology group $H_1(\alb_Y): H_1(Y,\Z)/\text{tors}\xrightarrow{H_1(\alpha)} H_1(W,\Z)\to H_1(\Alb_Y,\Z)$ is an isomorphism. In order to establish (ii), we first notice the following lemma essentially due to J. Stallings (see \cite[Theorem 5.1]{Sta65}):
\begin{lemma}[{\cite[Lemme 2.3]{Cam95}}]
\label{lemma:Stallings}
Let $\phi: K\to L$ be a morphism of finite connected cell complexes. Assume that $H^2(\phi): H^2(L,\Q)\to H^2(K,\Q)$ is injective, then $H_2(\phi_\ast):H_2(\pi_1(K),\Q)\to H_2(\pi_1(L),\Q)$ is surjective.
\end{lemma}
\begin{proof}
Note that we have the following commutative diagram:
\begin{center}
\begin{tikzpicture}[scale=3.0]
\node (A) at (0,0) {$H_2(L,\Q)$};
\node (A1) at (1,0) {$H_2(\pi_1(L),\Q)$,};
\node (B) at (0,1) {$H_2(K,\Q)$};
\node (B1) at (1,1) {$H_2(\pi_1(K),\Q)$};
\path[->,font=\scriptsize,>=angle 90]
(B) edge node[left]{$H_2(\phi)$} (A)
(B1) edge node[right]{$H_2(\phi_\ast)$} (A1);
\path[->>]
(A) edge (A1)
(B) edge (B1);
\end{tikzpicture}  
\end{center}
where the horizontal arrows are constructed above and they are surjective. By our assumption, the left arrow $H_2(\phi): H_2(K,\Q)\to H_2(L,\Q)$ is surjective, thus by 5-lemma, so is the right arrow $H_2(\phi_\ast)$.   
\end{proof}

With the lemma, above, we see that (ii) follows immediately from the injectivity of $H^2(\alpha): H^2(W,\Q)\to H^2(Y,\Q)$, which results from the more general {\hyperref[lemma:Kahler-cohomology]{Lemma \ref*{lemma:Kahler-cohomology}}} below. Thus we complete the proof of {\hyperref[thm:Campana]{Theorem \ref*{thm:Campana}}}.
\end{proof}

\begin{lemma}[cf.~{\cite[Lemme 2.4]{Cam95}}]
\label{lemma:Kahler-cohomology}
Let $\alpha: X\to Y$ be a surjective proper morphism between (not necessarily compact) connected complex manifolds, and assume that $X$ is K\"ahler. Then $H^i(\alpha): H^i(Y,\R)\to H^i(X,\R)$ is injective for every $i\in\Z_{\geqslant 0}$.
\end{lemma}
\begin{proof}
The idea of this result has already appeared in A. Fujiki's work \cite[Proof of Proposition 1.6]{Fuj78}. Let us remark that the compactness of $X$ (and of $Y$) is not necessary as long as we assume the morphism $\alpha$ is proper. Take a K\"ahler form $\omega$ on $X$, and set $r:=\dim X-\dim Y$. Let $Y_0$ be the Zariski open of $Y$ over which $\alpha$ is smooth, then we claim that the integral $c(y):=\int_{X_y} \omega|_{X_y}^r$ is independent of $y\in Y_0$. Indeed, it suffices to show $c(\cdot)$ is locally constant, hence by Ehresmann's theorem (see \cite[Proposition 9.3, p.209]{Voi02}) we can assume that $X_0:=\alpha^{-1}(Y_0)$ is diffeomorphic to a product $Y_0\times F$ where $F$ is a general fibre of $\alpha$. Then we can write $c(y)=\int_F\tau^\ast\omega|^r_{\{y\}\times F}$ where $\tau:Y_0\times F\xrightarrow{\simeq} X_0$ is the diffeomorphism given by Ehresmann's theorem, hence by $d$-closedness of $\omega$ we have
\[
dc(y) = \int_F d(\tau^\ast\omega|^r_{\{y\}\times F})=0.
\]
The claim is thus proven, and we simply denote this constant by $c$. Then for any real $2\dim Y$-form $\phi$ with compact support on $Y$, we have 
\[
\int_X\alpha^\ast\phi\wedge\omega^r=\int_{X_0}\alpha^\ast\phi\wedge\omega^r=c\cdot\int_{Y_0}\phi=c\cdot\int_Y\phi.
\]
Now take $[u]\in\ker(H^i(\alpha))$, then $\alpha^\ast u$ is $d$-exact, hence for any $[v]\in H^{2\dim Y-i}_c(Y,\R)$ we have
\begin{align*}
0 &=\int_X\alpha^\ast(u\wedge v)\wedge\omega^r=c\int_Y u\wedge v,\\
 & \uparrow  \\
 & \text{\tiny by Stokes} 
\end{align*}
thus $[u]=0$ by Poincar\'e duality.
\end{proof}

As a corollary of {\hyperref[thm:Campana]{Theorem \ref*{thm:Campana}}}, we have the following result, which is nothing but a refinement of {\hyperref[prop:Alb_surj_pi1]{Proposition \ref*{prop:Alb_surj_pi1}}}.
\begin{corollary}[{\cite[Corollaire 3.1]{Cam95}}]
\label{cor:Campana}
Let $Y$ be a compact K\"ahler manifold and set $G:=\pi_1(Y)$. Assume that the Albanese map of $Y$ is surjective. Then 
\begin{itemize}
\item[\rm(a)] $f:=\alb_{Y\ast}:G\to\pi_1(\Alb_Y)$ is surjective.
\item[\rm(b)] $G'_1=G'_n=G'_\infty$ for any $n\geqslant1$, and $G^{\nilp}\simeq\pi_1(\Alb_Y)$.
\end{itemize}
\end{corollary}

Before giving the proof of the corollary, let us recall the following well-known result:
\begin{lemma}[{\cite[Proposition 1.3]{Cam91}, \cite[Lemma 1.2(i)]{Voi21}}]
\label{lemma:pi1-proper}
Let $f:X\to Y$ be a proper surjective morphism between complex varieties, and assume that $Y$ is normal. Then $f_\ast\pi_1(X)$ has finite index in $\pi_1(Y)$.
\end{lemma}
\begin{proof}
By taking a resolution of $X$, we see clearly that it suffices to prove the lemma for $X$ smooth. In this case, by generic smoothness there is a Zariski open $Y_0\subseteq Y$ such that $f$ is a smooth morphism (holomorphic submersion) over $Y_0$\,. Set $X_0:=f^{-1}(Y_0)$, then by Ehresmann's theorem (\cite[Proposition 9.3, p.209]{Voi02}) $f_0:=f|_{X_0}:X_0\to Y_0$ is topological fibre bundle, then by looking at the homotopy sequence for $f_0$ we see that $f_{0\ast}\pi_1(X_0)$ has finite index in $\pi_1(Y_0)$ (any fibre of $f_0$ is compact, thus has only finitely many connected components, i.e. $\#\pi_0<+\infty$). In addition, we have the following commutative diagram
\begin{center}
\begin{tikzpicture}[scale=2.5]
\node (A) at (0,0) {$\pi_1(X)$};
\node (A1) at (1,0) {$\pi_1(Y)$,};
\node (B) at (0,1) {$\pi_1(X_0)$};
\node (B1) at (1,1) {$\pi_1(Y_0)$};
\path[->,font=\scriptsize,>=angle 90]
(A) edge node[below]{$f_\ast$} (A1)
(B) edge node[above]{$f_{0\ast}$} (B1);
\path[->>]
(B) edge (A)
(B1) edge (A1);
\end{tikzpicture}  
\end{center}
where the vertical arrows are induced by the inclusions, which are surjective by \cite[0.7(B)]{FL81}. Hence $f_\ast\pi_1(X)$ has finite index in $\pi_1(Y)$.

\end{proof}


\begin{proof}[Proof of {\hyperref[cor:Campana]{Corollary \ref*{cor:Campana}}}]
By virtue of {\hyperref[thm:Campana]{Theorem \ref*{thm:Campana}}}, it suffices to establish (a). Since $\alb_Y$ is surjective, from {\hyperref[lemma:pi1-proper]{Lemma \ref*{lemma:pi1-proper}}} we know that $f$ is of finite index $d$. Let $h: T\to\Alb_Y$ be an isogeny of degree $d$, such that $h_\ast(\pi_1(T))=f(G)$, then by the lifting lemma we get a factorization $\beta: Y\to T$ such that $\alb_Y=h\circ\beta$; from the universal property of the Albanese map, $h$ is a fortiori an isomorphism, and $f=\alb_{Y\ast}$ is thus surjective.   
\end{proof}

Finally let us prove {\hyperref[thm:main2]{Theorem \ref*{thm:main2}}}. Let $\alb_X: X\dashrightarrow \Alb_X$ be the Albanese map (of any desingularization) of $X$, then  since $X$ has rational singularities by \cite[Lemma 8.1]{Kaw85} $\alb_X$ is an everywhere defined morphism, such that $\alb_{X'}=\phi\circ\alb_X$ for any desingularization $\phi: X'\to X$ of $X$. From \cite[Corollary 2]{Zha05} we see that $\alb_X$, and thus $\alb_{X'}$\,, are algebraic fibre spaces, then we can apply {\hyperref[prop:Alb_surj_pi1]{Proposition \ref*{prop:Alb_surj_pi1}}} (or {\hyperref[cor:Campana]{Corollary \ref*{cor:Campana}}}) to $X'$ to conclude that the torsion-free nilpotent completion of $G:=\pi_1(X')\simeq\pi_1(X)$ is Abelian, here the isomorphism $\pi_1(X')\simeq\pi_1(X)$ follows from \cite[Theorem 1.1]{Tak03}; but by {\hyperref[thm:main1]{Theorem \ref*{thm:main1}} $G$ itself is already virtually nilpotent, thus it is almost Abelian, this completes the proof of {\hyperref[thm:main2]{Theorem \ref*{thm:main2}}.  


==> old-ref.tex <==
\begin{thebibliography}{99} 

\bibitem{Cam95} Campana, Fr\'ed\'eric, {\em Remarque ssur les groupes de Kähler nilpotents}, Ann. Sci. \'E.N.S, 28 (1995), no.3, 307--316 
\bibitem{CC}Cheeger, J and Colding, T.H {\em Lower bounds on Ricci curvature and the almost rigidity of warped
products}, Ann. of Math. 144 (1996), no. 1, 189-237
\bibitem{CCHSTT} Chen, Y., Chiu, S., Hallgren, M., Szekelyhidi, G., To, D. and Tong, F. {\em   On K\"ahler-Einstein Currents}, arXiv:2502.09825

\bibitem{DPS} Demailly, J.-P., Peternell, T.  and Schneider,  M. {\em Kahler manifolds with numerically effective Ricci class}, Camp. Math., 89, 1993,  p. 217--240

\bibitem{De} Demailly, J.P. {\em Analytic methods in algebraic geometry}, https://www-fourier.ujf-grenoble.fr/~demailly/manuscripts/analmeth.pdf 

\bibitem{DSZZ} Deng, Q., Santos-Rodríguez, J.,   Zamora, S. and  Zhao, X. {\em Margulis lemma on RCD(K,N) spaces},  arXiv:2308.15215

 \bibitem{EGZ} Eyssidieux, P.,   Guedj, V. and Zeriahi, A. {\em Singular
K\"{a}hler-Einstein metrics}, J. Amer. Math. Soc. 22 (2009),
607--639

\bibitem{FGS}  Fu X., Guo, B. and Song, J.  {\em  RCD structures on singular Kahler spaces of complex dimension three}, arXiv:2503.08865

\bibitem{Fuj78} Fujiki, Akira, {\em On automorphism groups of compact K\"ahler manifolds}, Invent. Math., 44 (1978), no.3, 225--258

\bibitem{GPSS1} Guo, B., Phong, D.H., Song, J.  and Sturm, J. {\em Sobolev inequalities on K\"ahler spaces}, 2023, arXiv:2311.00221

\bibitem{GPSS2}Guo, B., Phong, D.H., Song, J.  and Sturm, J.  {\em Diameter estimates in K\"ahler geometry},  {Comm. Pure Appl. Math.}, Volume 77, Issue 8 (2024), 3520--3556

\bibitem{GPSS3}Guo, B., Phong, D.H., Song, J.  and Sturm, J.   {\em Diameter estimates in K\"ahler geometry II: removing the small degeneracy assumption}, Math. Z. 308, 43 (2024) 
\bibitem{GS} Guo, B. and Song, J. {\em Nash entropy, Calabi energy and geometric regularization of singular K\"ahler metrics}, arXiv:2502.02041

\bibitem{GKB}Greb, D., Kebekus, S., and Peternell, T. {\em
Singular spaces with trivial canonical class}, Minimal models and extremal rays (Kyoto, 2011), 67–113.
Adv. Stud. Pure Math., 70 Mathematical Society of Japan, [Tokyo], 2016

\bibitem{Ho}Honda, S. {\em Bakry-\`Emery conditions on almost smooth metric measure spaces}, Anal. Geom. Metr. Spaces 6 (2018), no. 1, 129--145
\bibitem{Kol}  Ko\l{}odziej, S. {\em The complex Monge-Amp\`ere equation}, Acta Math. 180 (1998) 69--117
\bibitem{Kollar} Kollár, J. {\em
Shafarevich maps and automorphic forms}, Princeton University Press, Princeton, NJ, 1995. x+201 pp
\bibitem{Kaw85} Kawamata, Yujiro, {\em Minimal models and the Kodaira dimension of algebraic fibre spaces}, J. für Reine Angew. Math., 363 (1985), 1--46 
\bibitem{KW} Kapovitch, V and Wilking, B {\em Structure of fundamental groups of manifolds with Ricci curvature
bounded below}, http://arxiv.org/abs/1105.5955 (2011)
\bibitem{LS1} Liu, G. and Sz\'ekelyhidi, G. {\em Gromov-Hausdorff limits of K\"ahler manifolds with Ricci curvature bounded below}, Geom. Funct. Anal. 32 (2022), no. 2, 236--279
\bibitem{Pau97} Paun, M. {\em Sur le groupe fondamental des varietes Kahleriennes compactes a classe de Ricci numeriquement effective}, C. R. Acad. Sci. Paris Sér. I Math. 324 (1997), no. 11, 1249--1254


\bibitem{Sta65} Stallings, John, {\em Homology and Central Series of Groups}, J. Alg., 2 (1965), no.2, 170--181

\bibitem{Tak03} Takayama, Shigegaru, {\em Local simple connectedness of resolutions of log-terminal singularities}, Int. J. Math., 14 (2003), no.8, 825--836

\bibitem{Voi02} Voisin, Claire, {\em Th\'eorie de Hodge et g\'eom\'etrie alg\'ebrique complexe}, Vol.10 Cours sp\'ecialis\'es, Paris: Soci\'et\'e math\'ematique de France, 2002

\bibitem{Zha05} Zhang, Qi, {\em On projective varieties with nef anticanonical divisors}, Math. Ann. 332 (2005), no.3, 697--703 

\end{thebibliography}
